Towards Stable Interstellar Flight: Levitation of a Laser-Propelled Sailcraft*

Exploring and traveling to distant stars has long fascinated humanity but has been limited due to the vast distances. The Breakthrough Starshot Program aims at eliminating this limitation by traveling to Alpha Centauri, which is 4.37 light-years away. Thus, it is only possible if a vehicle travels at a substantial fraction of the speed of light. The Breakthrough Starshot Program initiatives to develop a proof-of-concept that is accelerating a sail to relativistic speeds using a laser beam aimed at the sail. At this high speed, while a stable beam riding is one of the crucial concerns of this concept, the dynamic stability analysis of a sail is hardly present in the previous literature. Furthermore, it is important to investigate the dynamic stability in the experiment before driving the sail to relativistic speeds. As a proof of concept, we study the dynamic stability of the sail levitated at a certain height by a laser beam. The sail's dynamics are modeled as a rigid body whose shape is parameterized by a sweep function. We estimate the region of attraction (ROA) for dynamic stability analysis using Lyapunov theory and Sum-of-square (SOS) programming. The ROA confirms how much a levitated sail can tolerate the transverse and angular perturbations. We also conclude on some of the important parameters of the sail that affects the dynamic stability. Simulation results validate our theoretical analysis.

==> levitation.tex <==
\section{Levitation of the Laser Beam-driven Sail}
	%
 	\subsection{Hypothetical Setup of the Experiment}
	For an experimental setup, we assume that a sail is placed in a vacuumed chamber and is driven by a Gaussian laser beam as discussed previously. We also assume that a velocometer acts like a sensor and can send the feedback signal to the actuator (laser)  to produce the force from the beam to levitate the sail. A hypothetical representation of the experiment is shown in Fig.\ \ref{fig:experiment}. 
	%
	\begin{figure}[h]
		\begin{center}
			\includegraphics[scale = 0.75]{fig/laser_driven-levitation.png}
			\caption{Schematic of a sub-scale experimental laser-driven sail. Credit: Breakthrough Foundation.}
			\label{fig:experiment}
		\end{center}
	\end{figure}
	%
	%
	%
	\subsection{Lyapunov Based Design}
	It turns out that we need to design a nonlinear closed-loop control law that not only can levitate the sail at an assigned height but also guarantees the closed-loop stability of the sail. In this case, the force directly drives the states $z$ and $v_z$ and the other states indirectly. Thus, the states $z$ and $v_z$ are considered as actuated states. The dynamics of the actuated system can be written as
	%
	\begin{subequations}\label{eq:1D}
		\begin{align}
			\dot{z} & = v_z,\\
			\dot{v}_z & = g + \frac{F_z}{M}, 
		\end{align}
	\end{subequations}
	%
	where $F_z$ is the $z$ component of the force $\textbf{F}$ given in Eq.\ \eqref{eq:force}. 
	%
	We can rewrite Eq.\ (\ref{eq:1D}) as,
	%
	\begin{equation} 
		\begin{bmatrix}  \dot{z} \\ \dot{v}_z 
		\end{bmatrix}= 
		\left[\begin{array}{c}
			v_z \\ g 
		\end{array}\right] + \begin{bmatrix}  0 \\ 	\frac{G_z}{M} 
		\end{bmatrix}u,
	\end{equation}
	%
	where,
	%
	\begin{subequations}
		\begin{align*}
			\textbf{G} & =   \frac{1}{ c \pi \sigma^2} (R_I^B)^{-1} \iint_{S(\Theta_1)}    e^{-\frac{ (x^2+y^2)}{ 2 \sigma^2}} \hat{\textbf{b}}. \hat{\textbf{n}}(\textbf{x})  \textbf{dS}, \\
			u & = P_0,
		\end{align*}
	\end{subequations}
	%
	and $G_z$ is the $z$ component of $\textbf{G}$. Note $F_x = G_x$, $F_y = G_y$, and $F_z = G_zu$. 
	%
	The actuator can only produce force along the $z$-direction but not any applied  torque.  But the torque due to the force $\textbf{F}$ is still considered. If there is any angular perturbation, \textit{i.e.}, $(R_I^B)^{-1} \ne I_3$, non-zero $x$ and $y$ components of $\textbf{F}$ will be produced.
	Moreover, we assume that spinning of the sail around the $z$-axis is allowed and will not affect the dynamic stability, but the spinning around $x$ and $y$ will as these spinnings will tumble the sail. We separate the actuated and underactuated states as
	%
	\begin{align*}
		\textbf{x}_a &= 	\begin{bmatrix} z & v_z	\end{bmatrix}^T,\\
		\textbf{x}_u &= \begin{bmatrix} x & y & \psi & \theta & \phi &
			v_{x} & v_{y} & \omega_x & \omega_y & \omega_z
		\end{bmatrix}^T.
	\end{align*}
	%
	Consider the Lyapunov function for the actuated states to design a closed-loop controller
	%
	\begin{equation} 
		V_a (\textbf{x}_a) = \frac{1}{2} z^2 + \frac{1}{2} v_z^2 
	\end{equation}
	%
	of which the time derivative is
	%
	\begin{align}
		\dot{V}_a  & = z v_z +v_z (g+\frac{G}{M} u).
	\end{align}transverse and angular perturbations
	%
	The control input 
	%
	\begin{equation} 
		u = P_0 =  \frac{-M}{G} [ g +  z + v_z]
	\end{equation}
	%
	leads to $\dot{V}_a = - v_z^2 <0$. If we want to levitate the sail at $z=z_d$, the transformation $e = z-z_d$ accommodates the case and we obtain
	%
	\begin{equation} 
		u = P_0 =  \frac{-M}{G} [ g+ e + v_z].
	\end{equation}
	%
	This feedback control law $u$ levitates the sail at $z_d$. Now we need to analyze the local stability of the internal dynamics. The internal dynamics can be written as,
	%
	\begin{subequations}\label{eq:internal}
		\begin{align}
			\dot{x} & = v_x, \dot{y}  = v_y,\\
			\dot{\boldsymbol{\alpha}} & = L^I_B \boldsymbol{\omega}_b, \\
			\dot{v}_x & = \frac{F_x}{M}, \dot{v}_y  = \frac{F_y}{M} , \\
			\dot{\boldsymbol{\omega}}_b & = J^{-1} [- \boldsymbol{\omega}_b^{X} \times J\boldsymbol{\omega}_b + \boldsymbol{\tau}_b].
		\end{align}
	\end{subequations}
	%
	As the sail is moving along $z$ axis and spinning around the $z$-axis is permitted, the states $\psi$ and $\omega_z$ can be excluded from the states' associated with the internal dynamics and the remaining states of the internal dynamics can be written as,
	%
	\begin{equation*} 
		\textbf{x}_u = \begin{bmatrix} x & y  & \theta & \phi &
			v_{x} & v_{y} & \omega_x & \omega_y 	\end{bmatrix}^T. 
	\end{equation*}
	%
	%The stability of the internal dynamics is analyzed by Lyapunov’s linearization theorem. 
	Linearizing the internal dynamics around $\textbf{x}_u = \textbf{0}$ leads to a linear system as follows:
	%
	\begin{equation}\label{eq:linear}
		\dot{\textbf{x}}_u(t) = A \textbf{x}_u,
	\end{equation} 
	%
	where
	%
	\begin{equation*}
		\begin{small}
			A = \begin{bmatrix} 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0\\ 
				0 & 0 & 0 & 0 & 0 & 1 & 0 & 0\\
				0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\\	 
				0 & 0 & 0 & 0 & 0 & 0 & 1 & 0\\
				A_1 & 0 & A_2 & 0 & A_6 & A_8 & 0 & 0\\
				0 & A_1 & 0 & -A_2 & -A_8 & A_7 & 0 & 0\\
				0 & A_3 & 0 &  A_4 & 0 & 0 & 0 & A_5\\
				-A_3 & 0 & A_4 & 0  & 0 & 0 & -A_5 & 0\\
			\end{bmatrix}_{\textbf{x}_u = \textbf{0}}
		\end{small},
	\end{equation*} 
	\\	
	\begin{doublespace}
		\noindent and $A_1 = \frac{1}{M} \frac{\partial F_x}{\partial x} = \frac{1}{M} \frac{\partial F_y}{\partial y}$, $A_2 = \frac{1}{M} \frac{\partial F_x}{\partial \theta} = - \frac{1}{M} \frac{\partial F_y}{\partial \phi}$, $A_3 = \frac{1}{J_x} \frac{\partial \tau_x}{\partial y} = -\frac{1}{J_y} \frac{\partial \tau_y}{\partial x}$, $A_4 = \frac{1}{J_x} \frac{\partial \tau_x}{\partial \phi} = \frac{1}{J_y} \frac{\partial \tau_y}{\partial \theta}$, $A_5 = \frac{J_x-J_z}{J_x}\omega_z$, $A_6 = -D_{11}/M$, $A_7 = -D_{22}/M$, $A_8 = -D_{12}/M$.
	\end{doublespace}
	%	
	Assume that the matrix $A$ is Hurwitz ($Re\{\lambda_i(A)<0\}$) for some selection of the parameter set $\Theta$ and the matrix $D$. The numerical simulations in the result section  suggest that this is indeed possible. We can find a local Lyapunov function (LLF) for the underactuated system as,
	%
	\begin{equation}\label{eq:lyap}
		V(\textbf{x}_u) = \textbf{x}_u^T P \textbf{x}_u,
	\end{equation} 
	for the system in Eq.\ \eqref{eq:linear} by solving the Lyapunov equation,
	%
	\begin{equation}\label{eq:lyapeq}
		PA + A^T P = - Q.
	\end{equation}
	%
	Note that, $\dot{V}(\textbf{x}_u) = - \textbf{x}_u^T Q \textbf{x}_u$. If $Q = I$ and $A$ is Hurwitz, $P$ is positive definite and unique. Hence, the linearized system in Eq.\ \eqref{eq:linear} is locally stable. This LLF is used to compute the ROA to study the dynamic stability of the sail.
	
	
	

